MetaPose: Fast 3D Pose from Multiple Views without 3D Supervision

In the era of deep learning, human pose estimation from multiple cameras with unknown calibration has received little attention to date. We show how to train a neural model to perform this task with high precision and minimal latency overhead. The proposed model takes into account joint location uncertainty due to occlusion from multiple views, and requires only 2D keypoint data for training. Our method outperforms both classical bundle adjustment and weakly-supervised monocular 3D baselines on the well-established Human3.6M dataset, as well as the more challenging in-the-wild Ski-Pose PTZ dataset.

==> 4_experiments_OLD.tex <==
\subsection{Teacher-student variant \TODO{ben}}
\color{red}
\input{figs/method/stage2}
\begin{itemize}
\item Then we iteratively refine this initial guess for the 3D pose and cameras via gradient decent over the likelihood given per-view per-joint localization heatmaps obtained using a single-view 2D pose estimation network.
\end{itemize}
\TODO{...}
\paragraph{Iterative refinement -- Stage 2}
During the second stage, illustrated in Figure~\ref{fig:fig2_method_stage2}, we use per-view heatmaps to refine the initial guess by solving (\ref{eq:main_objective}) via gradient decent starting from the initial guess acquired on the previous stage.
We refer to the resulting pose and cameras estimate $(p_{\text{ref}}, c_{\text{ref}})$ as a ``refined guess''.
\TODO{...}
% \paragraph{Fast Inference} 
% Note, during inference we only need to perform rigid alignment over per-view 3D estimates (Stage 1) to acquire an initial guess, and apply the neural optimizer $f_{\theta}$ to this guess in a feed-forward manner (Stage 3), no iterative refinement (Stage 2) is necessary. We provide pseudo-code for both training and inference in Supp.~\ref{sec:sup_pseudo}.
\TODO{...}
Similarly in spirit to the Deep Inverse Solver~\cite{ma2020deepoptimizer}, \TODO{...}
\TODO{should we mention the differences from \cite{ma2020deepoptimizer} here? want to avoid the \textit{incremental contribution} bs...} \BU{re Deep Inverse Solver: in fact, without the teacher loss, our current model is not really ``similar in spirit'' anymore - we are just training a network to do normal ``reprojection error minimization'' starting from the EpiPolar pose init.}
\color{black}

\section{Experiments}\label{sec:experiments}

In this section, we specify datasets and metrics we used to validate the performance of the proposed method and a set of baselines and ablation experiments we conducted to evaluate the improvement in error provided by each stage and each supervision signal.

\paragraph{Data} 
We evaluated our method on Human3.6M \cite{ionescu2013human36m} (H36M) dataset with four fixed cameras and a more challenging SkiPose-PTZ \cite{rhodin2018skipose} (SkiPose) dataset with six \textit{moving} pan-tilt-zoom cameras. We used standard train-test evaluated protocol for H36M \cite{iskakov2019learnable,kocabas2019epipolar} with subjects 1, 5, 6, 7, and 8 used for training, and 9 and 11 used for testing. We additionally pruned the H36M dataset by taking each 16-th frame from it, resulting in 24443 train and 8516 test examples, each example containing information from four cameras. We evaluated our method on two subsets of SkiPose: the ``full'' dataset used by \citet{rhodin2018skipose} (1315 train / 284 test), and a ``clean'' subset (1035 train / 230 test) used by \citet{wandt2020canonpose} that excludes 280 examples with visibility obstructed by snow, each example containing information from six cameras. 
% We additionally augment the SkiPose dataset by randomly shuffling camera order during training to prevent the neural optimizer from overfitting on the small training set. 
In each dataset, we used the first 64 examples from the train split as a validation set.

\paragraph{Metrics}
We report Procrustes aligned Mean Per Joint Position Error (PMPJPE) that measures the L2-error of 3D joint estimates after applying the optimal rigid alignment to the full predicted 3D pose and the ground truth 3D pose, and therefore ignores the overall pose orientation error, as well as the Normalized Mean Per Joint Position Error (NMPJPE) that measures the error after optimally scaling and shifting the prediction for the given camera frame to the ground truth pose in that camera frame, so it is sensitive to the pose orientation, but ignores the errors in ``scale''. We do not report the non-normalized pose estimation error because, in the absence of intrinsic camera parameters, the correct absolute scale can not be estimated from data. We additionally report the amount of time ($\Delta t$) it takes to perform multi-view 3D pose inference using different methods.

\input{tables/results_h36m}
\input{tables/results_ski}

\paragraph{Baselines} 
On H36M we lower-bound the error 
% of our model 
with the state-of-the-art fully-supervised baseline of \citet{iskakov2019learnable} that uses ground truth camera parameters to aggregate multi-view predictions during inference. We also compare the performance of our method to methods that use multi-view 2D supervision during training but only perform inference on a single view at a time: self-supervised EpipolarPose (EP) \cite{kocabas2019epipolar} and CanonPose (CP) \cite{wandt2020canonpose}, as well as the weakly supervised baselines of \citet{iqbal2020weakly} and \citet{rhodin2018skipose}. We applied EpipolarPose to our own set of human bounding boxes on H36M, so our per-view results differ from those reported by \citet{kocabas2019epipolar}. On SkiPose we compared our model with the only two baselines available in the literature: CanonPose \cite{wandt2020canonpose} and \citet{rhodin2018skipose}. CanonPose is preferable to EpipolarPose on the SkiPose dataset because it does not assume fixed cameras. We include results on both the ``clean'' and ``full'' subsets of SkiPose (described previously) for completeness; however CanonPose was trained and evaluated only on the ``clean'' subset, so in the absence of monocular 3D methods trained and evaluated on the ``full'' SkiPose dataset, for the sake of completeness, we trained and evaluated our method using ground truth data with Gaussian noise in place of CanonPose predictions, \textit{only} when evaluating \textit{on that subset} (``full'') of SkiPose.
% \AT{how to prevent reviewers from attacking here?}

We also compared our method against ``classical'' bundle adjustment initialized with ground truth extrinsic camera parameters, and fixed ground truth intrinsic parameters of all cameras, therefore putting it into unrealistically favorable conditions. We used the well-tested implementation of bundle adjustment in AniPose \cite{karashchuk2020anipose} that uses an adapted version of the 3D registration algorithm of \citet{zhou2016fast}. This approach takes point estimates of joint locations as an input (i.e. no uncertainty) and iteratively refines camera parameters and joint location estimates. 

% In addition to metrics mentioned in the previous paragraph, we compare methods based on whether they were 1) trained with full 3D supervision, 2D supervision, were self-supervised, or used a combination of 2D and 3D data, 2) whether they can aggregate multi-view data during inference, and if so 3) whether they can use joint uncertainty estimates produced by single-view methods (i.e. heatmaps). 

% Our findings are summarized in Tables~\ref{tab:h36m} and \ref{tab:ski}, and discussed in detail in Section~\ref{sec:results}.
% \AT{isn't having half the description here, half in Section~\ref{sec:results} a bit inconvenient?}

% Anrea: 
% \TODO{move questions to 5-results}
% \endinput
% I will do that next

\paragraph{Ablation experiments} 
We additionally measured different sources of remaining error in our predictions
% on Human3.6M and SkiPose datasets
by replacing each component discussed in Section~\ref{sec:method}
% and illustrated in Figure~\ref{fig:fig2_method} 
with either its ground truth equivalent or a completely random guess, as well as constraining supervision signals we pass to the neural optimizer. More specifically, we measured the effect of 1) varying the number of cameras used for training and evaluation; 2) priming different refinement methods with random and ground truth initialization; 3) using ``fake heatmaps'' centered around ground truth joints projected back into the image plane using different camera models; and 4) disabling and enabling losses and priors when training our neural optimizer. We did not measure the performance of the neural optimizer primed with the ground truth initialization because that would have just shown the ability of the neural network to approximate the identity function. 

%  (\ref{row:ani_pred_ht_ep_init},\ref{row:gd_pred_ht_ep_init}).  
% (Table~\ref{tab:ablation_h36m}; rows \ref{row:ani_pred_ht_rand_init} and \ref{row:gd_pred_ht_rand_init})

% We also estimated how much we gained by using such initialization by comparing to a completely random 3D pose and camera initialization (Table~\ref{tab:ablation_h36m}; rows \ref{row:ani_pred_ht_rand_init} and \ref{row:gd_pred_ht_rand_init})
 
% vs exact ground truth initialization. We also measured how much error is due to the \textit{imperfect heatmaps} by replacing predicted heatmaps with ``ground truth heatmaps'' centered around each joint projection with fixed small variance (rows \ref{row:ani_pred_ht_gt_init} vs \ref{row:ani_gt_ht_gt_init}, \ref{row:gd_gt_ht_ep_init}). We also checked how much error is due to the \textit{imperfect camera model} used during refinement by comparing results with ``full-projection ground truth heatmaps'' (default) vs ``weak-projected ground truth heatmaps'' obtained by projecting each node with correct weak camera parameters. We also measured much we gained by \textit{providing exact refinement results to the neural optimizer} the importance of providing good initial guess and ``exact solution'' to the neural optimizer to check whether it is necessary to prime it with good initial guess, and whether it is important to train it with ``known exact solution'' or it could find them itself. 

\paragraph{Architecture}
For monocular 2D pose estimation, we used the stacked hourglass network \cite{newell2016stacked} pre-trained on COCO pose 
% \AT{lowercase "pose"?} 
dataset \cite{guler2018densepose}. 
% We additionally trained a linear regression adapter to convert between COCO and H36M label formats (see supplementary Figure~\ref{fig:fig_label_formats} for labeling format comparison; this yielded better generalization then fine-tuning the pre-trained network on H36M directly, as shown in supplementary Table~\ref{tab:mono_data}). The COCO-pretrained network generalized very poorly to SkiPosePTZ dataset (see supplementary Figure~\ref{fig:fig_ski_hourglass}) because of the visual domain shift, so we fine-tuned the stacked hourglass network using ground truth 2D labels.
For monocular 3D estimation in Stage 1, we applied EpipolarPose \cite{kocabas2019epipolar} on Human3.6M and CanonPose \cite{wandt2020canonpose} on SkiPosePTZ. % There methods were self-supervised by networks trained on MPII % dataset, trained using PoseNet \todocitesome and AlphaPose \todocitesome respectively.
We note that differences in the joint labeling schemes used by these monocular 3D methods and our evaluation set do not affect the quality of \textit{camera} initialization we acquire via rigid alignment, as long as monocular 3D estimates for all views follow the same labeling scheme. 
Similar to prior work \cite{ma2020deepoptimizer}, each ``neural optimizer step'' is trained separately, and stop gradient is applied to all inputs. We used the same architecture across all experiments: $L$ fully-connected 512-dimensional layers followed by a fully-connected 128-dimensional, all with selu 
% \AT{check not SeLU, and why did you use them?} 
nonlinearities \cite{klambauer2017selu}, followed by a dense output of the size corresponding to the optimization space (flattened 3D pose and weak camera model parameters). We re-trained each stage multiple times until the \textit{validation} PMPJPE improved or we ran out of ``stage training attempts''. 
% We used a fully-connected neural network (with three-to-five layers depending on the setup and the dataset size) to parameterize each the neural optimizer step $f_{\theta}$. 
We refer our readers to Section~\ref{sec:sup_arch} in supplementary for a more detailed description of all components we used to train our neural optimizer and their reference performance on train and test. 

% We would like to mention that we used EpipolarPose \cite{kocabas2019epipolar} on H36M  and CanonPose \cite{wandt2020canonpose} on SkiPosePTZ. % There methods were self-supervised by networks trained on MPII % dataset, trained using PoseNet \todocitesome and AlphaPose \todocitesome respectively.
% We would like to note that, despite the significant shift in the labeling format between predictions of these monocular 3D methods and the format used in datasets we used for evaluation, this does not affect the quality of camera initialization we acquired via rigid alignment. We re-trained each stage multiple times until the \textit{validation} PMPJPE improved or we ran out of ``stage training attempts''. 

==> 5_results_OLD.tex <==
\section{Results}
\label{sec:results}

% Andrea's plan:
% \subsection{State-of-the-art}
% Mostly about 

% \subsection{Ablation and analysis}

% \todo{We additionally measured different sources of error
% % on Human3.6M and SkiPose datasets
% by replacing each component discussed in Section~\ref{sec:method}
% % and illustrated in Figure~\ref{fig:fig2_method} 
% with either its ground truth equivalent or a completely random guess, as well as constraining supervision signals we pass to the neural optimizer.
% Our findings are summarized in Tables~\ref{tab:ablation_h36m} and \ref{tab:ablation_ski}, and discussed in more detail in Section~\ref{sec:results}.
% \AT{isn't having half the description here, half in Section~\ref{sec:results} a bit inconvenient?}
% Below we describe the setup and the intention behind each experiment:}

% \paragraph{Effect of \# cameras}
% We checked how the pose estimation error is affected by the \textit{number of cameras} used for training and inference. dskajdklas jdklasjd klasjdakjdld ja
% see Table1. rows (3,4)

% \paragraph{Random vs. learnt guess (Stage\#1)}
% We estimated how much the \textit{initial guess} we acquire at stage 1 \textit{helps the refinement} compared to a random init.

\noindent
Our experiments lead us to the following observations.
In what follows, ``(\rref{ablation_h36m}{ani_pred_ht_gt_init})'' stands for ``Table \ref{tab:ablation_h36m}, row \#\ref{row:ani_pred_ht_gt_init}''.

\paragraph{State-of-the-art performance -- Tables~\ref{tab:h36m} and \ref{tab:ski}}
In terms of both PMPJPE and NMPJPE, our neural optimizer, primed with outputs of EpipolarPose (EP) on H36M and CanonPose (CP) on SkiPose, outperforms the bundle-adjustment baseline (AniPose \cite{karashchuk2020anipose}) initialized with ground truth (GT) by +35mm on H36M with four cameras and +2mm on SkiPose with six cameras.
% while simultaneously allowing for faster inference
Our method also outperforms weakly-supervised baselines by +13mm on H36M and by +30mm on SkiPose. It also outperforms the iterative refiner that was used to ``teach it'' by 3-5mm on H36M, while being 10x faster than the iterative refiner.

\paragraph{Few-camera performance}
On both H36M and SkiPose, the improvement over the bundle-adjustment baseline (AniPose \cite{karashchuk2020anipose} initialized with GT) increases to more then +100mm as the number of cameras used for training and inference decreases to just two (\rref{ablation_h36m}{ani_pred_ht_gt_init} vs \rref{ablation_h36m}{neur_pred_ht_ep_init}; \rref{ablation_ski}{ski_ani_sub_2d_gt} vs \rref{ablation_ski}{ski_our_sub_2d_can_fwd}).

\paragraph{Self-supervised performance}
On H36M, the neural optimizer is able to learn in a \textit{self-supervised fashion} -- using heatmap log-probability loss alone \textit{without} 2D ground truth supervision, and still outperform the iterative refiner that uses the same initial guess (\rref{ablation_h36m}{gd_pred_ht_ep_init} vs \rref{ablation_h36m}{neur_pred_ht_ep_init_logp_only}). On a smaller SkiPose dataset, self-supervised training fails (\rref{ablation_ski}{ski_our_sub_2d_can_logp}).
% \paragraph{Iterative refinement vs neural refinement}
% Refining the initial guess using single-view heatmaps (Stage 2) improves the error by 30-40mm (), 

% \vfill
% \TODO{and so on and so forth, this was a ``mock''}

% \begin{enumerate}[wide, labelwidth=!, labelindent=0pt,itemsep=-0.3ex,topsep=0.2ex]
% \item 
% \end{enumerate}

\paragraph{Analysis} We hypothesize that the \textit{weakly-supervised} neural optimizer was able outperform the iterative refiner by learning to compensate for the errors in other pre-trained components using ground truth 2D joint locations in the reprojection loss, since removing the reprojection loss decreases its performance (\rref{ablation_h36m}{neur_pred_ht_ep_init} vs \rref{ablation_h36m}{neur_pred_ht_ep_init_xopt_only}). We believe that the finite-capacity neural optimizer additionally regularizes the pose estimation problem, allowing the \textit{self-supervised} neural optimizer to outperform the iterative refiner that minimized the very same loss log probability loss (\rref{ablation_h36m}{gd_pred_ht_ep_init} vs \rref{ablation_h36m}{neur_pred_ht_ep_init_logp_only}). This also hints at why the analogous setup fails on SkiPose -- the smaller number of training examples led to overfitting and, consequently, poor performance on test. This also agrees with the measured discrepancy between train and test errors on SkiPose (Supp.~\ref{sec:extended_train_test_scores}). See Supp \ref{sec:supp_images} for qualitative examples of poses output at Stages 1-3. 
% \paragraph{Ablation experiments}

\subsection{Ablations} We additionally studied the sources of remaining error (40mm on H36M and 48mm on SkiPose).
%We replaced each component with their ground truth and random counterparts:
% \begin{enumerate}[wide, labelwidth=!, labelindent=0pt,itemsep=-0.3ex,topsep=0.2ex]

\paragraph{Heatmap error} 
We performed iterative refinement on ``fake'' heatmaps centered around reprojected ground truth joint locations  (\rref{ablation_h36m}{gd_pred_ht_ep_init} vs \rref{ablation_h36m}{gd_gt_ht_ep_init}; \rref{ablation_ski}{ski_gd_sub_2d_can} vs \rref{ablation_ski}{ski_gd_sub_gt_can}). This reveals that imperfections in \textit{heatmaps} generated by the 2D pose estimation network $f_{\text{2D}}$ contribute to at least 20mm error on both H36M and SkiPose across all views. Moreover, poor performance of the iterative refinement \textit{with ground truth heatmaps} in the two-camera setup on SkiPose hints at why AniPose fails in that setting -- first two cameras are too close relative to the distance to subjects (see Figure 4 in \citet{rhodin2018skipose}), rendering this problem ill-defined.

\paragraph{Camera model}
We also performed refinement on ``fake'' heatmaps centered around \textit{weakly} projected 3D locations of joints. This revealed that a \textit{weak camera model} used in our method contributes to at least 10mm-15mm of error on H36M (\rref{ablation_h36m}{gd_gt_ht_ep_init}-\rref{ablation_h36m}{gd_wgt_ht_gt_init}) and no error on SkiPose (\rref{ablation_ski}{ski_gd_sub_gt_can} vs \rref{ablation_ski}{ski_gd_sub_weak_gt_can}).

\paragraph{Initialization} We primed AniPose \cite{karashchuk2020anipose} and our iterative refiner with ground truth and random initial guesses. This reveals that both AniPose and iterative refinement fail to converge to a good solution without a \textit{good initialization} (\rref{ablation_h36m}{ani_pred_ht_rand_init}, \rref{ablation_h36m}{ani_gt_ht_rand_init}, \rref{ablation_h36m}{gd_pred_ht_rand_init}), but a ``perfect'' initialization only improves their error by additional 3-5mm (\rref{ablation_h36m}{gd_pred_ht_rand_init} vs \rref{ablation_h36m}{gd_pred_ht_gt_init}), so the initialization we get from Stage 1 is already ``good enough''. We also primed our \textit{neural optimizer with random initial guesses} (both during training and inference). This reveals that, when provided with enough training data (H36M) and enough cameras, our simple neural optimizer was able to quickly (in 3-5 steps) converge to a high-quality solution, only 3-5mm worse then when primed with outputs from Stage 1 (\rref{ablation_h36m}{neur_pred_ht_ep_init} vs  \rref{ablation_h36m}{neur_pred_ht_rand_init}). Moreover, when the training set is too small (SkiPose) random initialization actually improves final results in the few-camera setup (\rref{ablation_ski}{ski_our_sub_2d_can_fwd} vs \rref{ablation_ski}{ski_our_sub_2d_rand_fwd}).
% \end{enumerate}

We conclude that the fully-supervised baseline of \citet{iskakov2019learnable} likely approaches the limits of what can be done with a weak camera model on H36M, and that further progress might come from better heatmaps and a better camera model. Good performance of \methodname~in the ill-defined two-camera setup (SkiPose), which improves even further when primed with a random initial guess, supports our hypothesis about MetaPose 
% working better then the iterative refinement because of the 
% additionally 
regularizing the ill-defined problem of few-camera pose estimation with a finite-capacity neural network. 

\paragraph{Design decisions}
The remaining experiments show that only
% provide the following observations about the design of the learned optimizer:
% \begin{enumerate}[wide, labelwidth=!, labelindent=0pt,itemsep=-0.3ex,topsep=0.2ex]
% \item Only 
the full model that used all proposed components (reprojection loss $\mathcal L_{\pi}$, teacher loss $\mathcal L_{\tau}$, and, optionally, bone length prior $\mathcal L_{\text{bone}}$) was able to keep the pose estimation error low with fewer cameras on both H36M (\rref{ablation_h36m}{neur_pred_ht_ep_init}-\rref{ablation_h36m}{neur_pred_ht_ep_init_bone}) and SkiPose datasets (\rref{ablation_ski}{ski_our_sub_2d_can}-\rref{ablation_ski}{neuropt_net2d_ep_bl_fwd_only}). 
% Bone length prior improved the error on both datasets, especially with fewer views (\rref{ablation_h36m}{gd_pred_ht_ep_init_bone}, \rref{ablation_h36m}{neur_pred_ht_ep_init_bone}).
% \item In most cases (except \rref{ablation_h36m}{neur_pred_ht_rand_init}, \rref{ablation_h36m}{neur_pred_ht_random_init_logp_only}, \rref{ablation_ski}{ski_our_sub_2d_rand_fwd}), the near-optimal performance was achieved with a single step of neural optimizer ($M=1$), and the remaining 2-3 steps gave only 1-3mm of improvement in test error (see Suppl. \todo{!}). 
% \end{enumerate}
% We conclude that our pose inference method does benefit from the inclusion of all proposed losses and additional pose priors, more so in the few-camera setting. Multi-stages training, on the other hand, provided significant improvement only \textit{in the absence of a good initialization} (Suppl. \todo{!}).

\input{tables/results_ablation}

% \TODO{we did not perform neural refinement with GT init because that would measure the ability of the network to learn an identity function}


% Our findings are summarized in Tables~\ref{tab:ablation_h36m} and \ref{tab:ablation_ski}, and discussed in more detail in Section~\ref{sec:results}.
% \AT{isn't having half the description here, half in Section~\ref{sec:results} a bit inconvenient?}
% Below we describe the setup and the intention behind each experiment:

% \begin{enumerate}[wide, labelwidth=!, labelindent=0pt,itemsep=-0.3ex,topsep=0.2ex]
%     \item We checked how the pose estimation error is affected by the \textit{number of cameras} used for training and inference.
%     \item We estimated how much the \textit{initial guess} we acquire at stage 1 \textit{helps the refinement} compared to a random init.
%     \item We estimated how much error on stage 2 is due to the \textit{imperfect initialization} by looking at how the error changes when stage 2 is primed with the ground truth initialization.
%     \item We estimated how much error in stage 2 and AniPose is due to \textit{imperfect heatmaps} by looking at how the error changes when we replace heatmaps predicted by the neural network with ``fake heatmaps'' containing ground truth joint locations with fixed small uncertainty.
%     \item We estimated how much error on stage 2 is due to the \textit{imperfect camera model} by looking at how the error changes when we use weak-projected 3D joint positions to generate ``fake ground truth heatmaps'' instead.
%     \item We estimated how much the initial guess \textit{initial guess} we acquire at stage 1 \textit{helps the neural optimizer} (stage 3) compared to priming it with random guesses.
%     \item We estimated how much the \textit{exact solution} we acquire at stage 2 \textit{helps the neural optimizer} (stage 3), or the neural optimizer alone can find it by minimizing the re-projection error or the log-probability directly via backpropagation.
%     \item We estimated how much the \textit{ground truth 2D re-projection loss} helps the \textit{neural optimizer} learn to compensate for errors in previous stages.
%     \item We estimated how much the \textit{bone length prior} helps the exact refinement and the neural optimizer.
% \end{enumerate}

==> figs/fig2_method.tex <==
\begin{figure*}
\begin{center}
% \fakegraphics{Similar to Figure 1 but .}
% <left> <lower> <right> <upper>
% \includegraphics[width=\linewidth,trim=0 2in 0.15in 0,clip]{imgs/ssmvp_fig2_v4.pdf}
\vspace{-0.23in}\includegraphics[width=\linewidth,trim=0 0.2in 0.4in 0]{imgs/ssmvp_fig2_v7_1.pdf}
\end{center}
\caption{
\textbf{Proposed method}.
\textit{(Best viewed in color).}
% \AT{implied by caption that talks about colors}
Our method requires three stages during training
% : acquiring an initial guess, performing exact refinement, and training a neural optimizer to approximate the exact refinement
. On \textbf{Stage 1} we form an \textit{initial guess} for the 3D pose and the cameras by taking the mean of rigid aligned 3D poses estimated from each RGB image using an external monocular 3D method \cite{kocabas2019epipolar,wandt2020canonpose}. On \textbf{Stage 2} we \textit{refine our initial pose and cameras} guesses by maximizing the likelihood of projected joint locations given heatmaps of 2D joint location probabilities predicted for each frame using an external network. On \textbf{Stage 3} we fit a \textit{neural optimizer} $f_{\theta}$ to predict the result of the iterative refinement and minimize the reprojection error with the ground truth, using the initial guess and joint heatmaps as an input. During inference we can use Stage 3 instead of Stage 2 which is much faster.
% \AT{shouldn't we use lexicographic order? (so stage 1 top-right}
% \AT{is the single-view pose estimate (really) in input to stage 2? (overview)}
% \TODO{TODO: color code heatmaps, the initial guess arrows and exact refinement arrow with same colors} \TODO{finish drawing stage 2}
% \TODO{figure needs to appear ABOVE Sec.3, had to turn the page a lot...}
% \TODO{need to mention that we skip stage 2 during inference!}
}
% 
% }
\label{fig:fig2_method}
\end{figure*}

==> figs/fign_alg.tex <==
\begin{algorithm}[ht]
\caption{MetaPose Training}\label{alg:train}
\begin{algorithmic}[1]
\Require{$f_{\text{2D}}: \bm{x} \mapsto \bm{h}$ - pre-trained 2D pose heatmap network; $f_{\text{M3D}}: \bm{x} \mapsto \bm{\tilde p}$ - pre-trained monocular 3D network; $\{(\bm{x}^{(t, c)}, \bm{q}^{(t, c)})\}_{t, c}^{T, C}$ - dataset; $\theta_0$ - initial parameters for the neural optimizer; $F$ - forward neural optimizer model}
\Ensure{$\theta^*$ - optimal parameters of the neural optimizer}
\For{$t \in [1\dots T]$}
    \For{$c \in [1\dots C]$}
        \State $\bm{\tilde p}^{(t, c)} = f_{\text{M3D}}(\bm{x}^{(t, c)})$
        \State $\bm{h} = f_{\text{2D}}(\bm{x}^{(t, c)})$
        \For{$k \in [1\dots K]$}
            \State $\bm{g}^{(t, c)}_k = \operatorname{FitSphericalGMM}(\bm{h}_k)$
        \EndFor
    \EndFor
    \State $\bm{p}_{\text{init}}, \{\bm{e}_{\text{init}}^{(c)}\} = \operatorname{RigidAlignment}(\bm{\tilde p}^{(t, c)})$ \Comment{S1}
    \State $\bm{y}_{\text{ref}} = \bm{p}_{\text{init}}, \{\operatorname{ReParam}(\bm{e}_{\text{init}}^{(c)})\}$
    \For{$i \in [0\dots \text{refinement steps}]$} \Comment{S2}
        \State $\mathcal L = \mathcal L_{\text{logp}}(\bm{g}^{(t, c)}, \pi(\bm{y}_{\text{ref}}))$
        \State $\bm{y}_{\text{ref}} = \bm{y}_{\text{ref}} - \eta \cdot (\partial \mathcal L) / (\partial \bm{y})$
    \EndFor
    \State $\bm{p}_{\text{ref}}, \{\bm{e}_{\text{ref}}^{(c)}\} = \operatorname{UnReParam}(\bm{y}_{\text{ref}})$
\EndFor
\Comment{S1 and S2 can be pre-computed and cached}
\For{$i \in [0\dots \text{train epochs}]$} \Comment{S3}
    \For{$t \in [1\dots T]$}
    \State $\bm{y}_{i}^{(t)} = F(\theta; \bm{y}_{\text{init}}^{(t)}, \bm{g}^{(t)}, \pi(\bm{y}_{\text{init}}^{(t)}))$
    \State $\mathcal L = \mathcal L_{\text{neur}}(\bm{y}_{i}^{(t)}, \bm{y}_{\text{ref}}^{(t)}, \bm{q}^{(t)})$
    \State $\theta = \theta - \eta \cdot (\partial \mathcal L) / (\partial \theta)$
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{MetaPose Inference}\label{alg:infer}
\begin{algorithmic}[1]
\Require{$f_{\text{2D}}, f_{\text{M3D}}, \theta^*, F$ from Algorithm~\ref{alg:train}; $\{(\bm{x}^{(t, c)})\}_{t, c}^{T', C}$ - unlabeled test dataset of size $T'$}
\Ensure{$\{\bm{y}^{(t)}\}_{t}^{T'} = \{(\bm{p}^{(t)}, \{\bm{e}^{(t, c)}\}_c^C)\}_t^{T'}$ - test predictions}
\For{$t \in [1\dots T']$}
    \For{$c \in [1\dots C]$}
        \State $\bm{\tilde p}^{(t, c)} = f_{\text{M3D}}(\bm{x}^{(t, c)})$
        \State $\bm{h} = f_{\text{2D}}(\bm{x}^{(t, c)})$
        \For{$k \in [1\dots K]$}
            \State $\bm{g}^{(t, c)}_k = \operatorname{FitSphericalGMM}(\bm{h}_k)$
        \EndFor
    \EndFor
    \State $\bm{p}_{\text{init}}, \{\bm{e}_{\text{init}}^{(c)}\} = \operatorname{RigidAlignment}(\bm{\tilde p}^{(t, c)})$ \Comment{S1}
    % \Comment{\textbf{Note:} no S2!}
\EndFor \Comment{no S2!}
\For{$t \in [1\dots T']$} 
    \State $\bm{y}_{\text{neur}}^{(t)} = F(\theta^*; \bm{y}_{\text{init}}^{(t)}, \bm{g}^{(t)}, \pi(\bm{y}_{\text{init}}^{(t)}))$ \Comment{S3}
\EndFor
\end{algorithmic}
\end{algorithm}

==> figs/overview.tex <==
\begin{figure}
\centering
\includegraphics[width=.9\columnwidth,trim=0 3.2in 6.5in 0,clip]{imgs/stages/overview_v2.pdf}
\vspace{-0em}
\caption{
\textbf{Overview}.
Our method requires two stages during training. 
During Stage 1 we form an \textit{initial guess} for the 3D pose and cameras using rough single-view camera-frame estimates of 3D poses predicted by an external network \cite{kocabas2019epipolar,wandt2020canonpose}. During Stage 2 we train a \textit{neural optimizer} to predict a 3D pose and camera configuration that minimize the re-projection loss wrt ground truth 2D joint locations using the initial guess formed at Stage 1 and joint localization probability heatmaps predicted by a different external network as an input.
} % \caption
\label{fig:overview}
\end{figure}

==> figs/stage2.tex <==
\begin{figure}
\begin{center}
% <left> <lower> <right> <upper>
\includegraphics[width=\linewidth,trim=0 2.9in 5.0in 0,clip]{imgs/stages/stage2.pdf}
\end{center}
\vspace{-10px}\caption{
\textbf{Iterative optimization 2}. We \textit{refine our initial pose and cameras} guesses by maximizing the likelihood (\ref{eq:main_objective}) of projected joint locations given heatmaps of 2D joint location probabilities predicted for each frame using an external single-view pose estimation network. \TODO{adjust}}
\label{fig:fig2_method_stage2}
\end{figure}

==> tables/results_ablation.tex <==
% \ownpage{
\begin{table}
\begin{center}
% \small
\vspace{-5px}
\inctabcolsep{-3.5pt} {
\begin{tabular}{lcccccccc}\toprule
\multicolumn{3}{c}{\textbf{Setup}} & \multicolumn{2}{c}{\textbf{Inputs}} & \multicolumn{3}{c}{\textbf{\# cam}} \\ 
\cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8}
\# & Method & Loss & 2D & init & 4 & 3 & 2 \\ \midrule
% h36m_anipose_cam1_{k}/v2/eval/
\rowlabel{row:ani_pred_ht_gt_init}* & AniPose & - & $f_{\text{2D}}$ & GT & 75 & 106 & 167 \\
% h36m_anipose_gt_init_gt_ht_cam1_{}
\rowlabel{row:ani_gt_ht_gt_init} & AniPose & - & GT & GT &  0.3 & 0.5 & 2.7 \\
\rowlabel{row:ani_pred_ht_rand_init} & AniPose & - & $f_{\text{2D}}$ & rand &  198 & 215 & 269 \\
% h36m_anipose_rand_init_gt_ht_cam1_
\rowlabel{row:ani_gt_ht_rand_init} & AniPose & - & GT & rand &  154 & 153 & 245 \\

\cmidrule(lr){1-8} % ----------------
% \addlinespace[0.7em]
% \cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8}
\rowlabel{row:avg_ep_init}* & Average & - & - & EP &  74 & 76 & 83 \\
\rowlabel{row:gd_pred_ht_ep_init}* & Iterative & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & EP &  45 & 53 & 55 \\
% h36m_opt_rand_init_cam1_4_opt_res
\rowlabel{row:gd_pred_ht_rand_init} & Iterative & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & rand & 248 & 322 & 419 \\
\rowlabel{row:gd_pred_ht_gt_init} & Iterative & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & GT &  42 & 49 & 48 \\
% h36m_opt_cam1_4_gt_ht_opt_res
\rowlabel{row:gd_gt_ht_ep_init} & Iterative & $\mathcal L_{\text{logp}}$ & GT & EP &  17 & 20 & 24 \\
\rowlabel{row:gd_gt_ht_gt_init} & Iterative & $\mathcal L_{\text{logp}}$ & GT & GT &  14 & 16 & 20 \\
\rowlabel{row:gd_wgt_ht_ep_init} & Iterative & $\mathcal L_{\text{logp}}$ & W-GT & EP &  4 & 6 & 18 \\
\rowlabel{row:gd_wgt_ht_gt_init} & Iterative & $\mathcal L_{\text{logp}}$ & W-GT & GT &  1.4 & 1.7 & 2 \\

\cmidrule(lr){1-8} % ----------------

\rowlabel{row:neur_pred_ht_ep_init}* & \methodname & $\mathcal L_{\pi}, \mathcal L_{y}$ & $f_{\text{2D}}$ & EP &  40 & 44 & 46 \\
\rowlabel{row:neur_pred_ht_rand_init} & \methodname & $\mathcal L_{\pi}, \mathcal L_{y}$ & $f_{\text{2D}}$ & rand &  43 & 47 & 47 \\
\rowlabel{row:neur_pred_ht_ep_init_fwd_only} & \methodname & $\mathcal L_{\pi}$ & $f_{\text{2D}}$ & EP & 31 & 40 & 51 \\
\rowlabel{row:neur_pred_ht_ep_init_xopt_only} & \methodname & $\mathcal L_{y}$ & $f_{\text{2D}}$ & EP & 47 & 53 & 57 \\
\rowlabel{row:neur_pred_ht_ep_init_logp_only} & \methodname & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & EP & 39 & 44 & 50 \\
\rowlabel{row:neur_pred_ht_random_init_logp_only} & \methodname & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & rand & 43 & 49 & 54 \\

\cmidrule(lr){1-8} % ----------------

% (xopt_fwd|bone)(.*?)/test
\rowlabel{row:gd_pred_ht_ep_init_bone} & Iterative & $\mathcal L_{\text{logp}}, \mathcal L_{\text{bone}}$ & $f_{\text{2D}}$ & EP & 41 & 44 & 46 \\
\rowlabel{row:neur_pred_ht_ep_init_bone} & \methodname & $\mathcal L_{\pi}, \mathcal L_{y}, \mathcal L_{\text{bone}}$ & $f_{\text{2D}}$ & EP & 39 & 42 & 44 \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-5px}\caption{\textbf{Extended results and ablation on H36M.} 
% We report PMPJPE (lower is better) on the test split of H36M as a function of 1) the method used for refinement
% % - AniPose, average of EpipolarPose (EP) predictions, exact refinement, or our neural optimizer; 
% 2) losses minimized during training; 3) the 2D inputs used for refinement 
% % - predictions of the pose estimation network, or ground truth joint locations projected with full (GT) and weak (W-GT) camera model; 
% 4) the initialization used to prime the refinement; and 5) the number of cameras used for training and inference. 
Results marked with an asterisk (*) are extended versions of main results reported in Table~\ref{tab:h36m}. \vspace{-10px}
% \TODO{numbers with ' might have improved for 1-5mm over time, need to check experiments again}
}
\label{tab:ablation_h36m}

% \end{table}

% \begin{table}

\begin{center}
% \small

% \inctabcolsep{-2pt} {
\inctabcolsep{-4pt} {
\begin{tabular}{lcccccccccc}\toprule
\multicolumn{4}{c}{\textbf{Setup}} & \multicolumn{2}{c}{\textbf{Inputs}} & \multicolumn{3}{c}{\textbf{\# cam}} \\ 
\cmidrule(lr){1-4} \cmidrule(lr){5-6} \cmidrule(lr){7-9}
\# & Method & Sub. & Loss & 2D & init & 6 & 4 & 2 \\ \midrule

\rowlabel{row:ski_ani_sub_2d_gt}*& AniPose & C & - & $f_{\text{2D}}$ & GT &  50 & 52 & 221 \\
\rowlabel{row:ski_avg_full_2d_can}* & Average & C & - & - & CP &  81 & 82 & 86 \\
\rowlabel{row:ski_gd_sub_2d_can}*& Iterative & C & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & CP & 31 & 35 & 78 \\
\rowlabel{row:ski_gd_sub_2d_gt}& Iterative & C & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & GT & 28 & 30 & 40 \\
\rowlabel{row:ski_gd_sub_gt_can}& Iterative & C & $\mathcal L_{\text{logp}}$ & GT & CP & 8 & 8 & 29 \\
\rowlabel{row:ski_gd_sub_weak_gt_can}& Iterative & C & $\mathcal L_{\text{logp}}$ & W-GT & CP & 8 & 7 & 28 \\
\rowlabel{row:ski_our_sub_2d_can}*& \methodname & C & $\mathcal L_{\pi}, \mathcal L_{y}$ & $f_{\text{2D}}$ & CP & 53 & 53 & 75 \\
% ski_canon_*_dense512x2_perm100_fwd_only
\rowlabel{row:ski_our_sub_2d_can_fwd}*& \methodname & C & $\mathcal L_{\pi}$ & $f_{\text{2D}}$ & CP &  48 & 45 & 55 \\
\rowlabel{row:ski_our_sub_2d_rand_fwd}& \methodname & C & $\mathcal L_{\pi}$ & $f_{\text{2D}}$ & rand & 51 & 48 & 53 \\
% ski_canon_cam1_6_perm100_logp/0311-2007 - wrong model size
% ski_canon_*_dense512x2_perm100_logp
\rowlabel{row:ski_our_sub_2d_can_logp}& \methodname & C & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & CP &  240 & 241 & 240 \\
% ski_canon_*_perm100_xopt_only
\rowlabel{row:ski_neur_net2d_rep_ep} & \methodname & C & $\mathcal L_{y}$ & $f_{\text{2D}}$ & CP & 55 & 53 & 89 \\

\cmidrule(lr){1-9} % ----------------
\rowlabel{row:gd_net2d_rep_ep} & Iterative & C & $\mathcal L_{\text{logp}}, \mathcal L_{\text{bone}}$ & $f_{\text{2D}}$ & CP & 27 & 29 & 34 \\
\rowlabel{row:neuropt_net2d_ep_bl} & \methodname & C & $\mathcal L_{\pi}, \mathcal L_{y}, \mathcal L_{\text{bn}}$ & $f_{\text{2D}}$ & CP & 50 & 49 & 58 \\
\rowlabel{row:neuropt_net2d_ep_bl_fwd_only} & \methodname & C & $\mathcal L_{\pi}, \mathcal L_{\text{bone}}$ & $f_{\text{2D}}$ & CP & 48 & 46 & 49 \\

\cmidrule(lr){1-9} % ----------------

\rowlabel{row:ski_ani_full_2d_gt}& AniPose & F & - & $f_{\text{2D}}$ & GT & 56 & 60 & 231 \\
\rowlabel{row:ski_avg_full_2d_nz} & Average & F & - & - & GT$+\varepsilon$ & 102 & 131 & 197 \\
\rowlabel{row:ski_gd_full_2d_nz}& Iterative & F & $\mathcal L_{\text{logp}}$ & $f_{\text{2D}}$ & GT$+\varepsilon$ & 32 & 41 & 134 \\
\rowlabel{row:ski_our_full_2d_nz}& \methodname & F & $\mathcal L_{\pi}, \mathcal L_{y}$ & $f_{\text{2D}}$ & GT$+\varepsilon$ &  48 & 52 & 73  \\

\bottomrule
\end{tabular}
}

\end{center}
\vspace{-5px}\caption{\textbf{Extended results and ablation on SkiPTZ.} 
% Notation is consistent with Table~\ref{tab:ablation_h36m}. 
% The first section (rows 1-7) show experiments on the ``clean'' (C) subset of SkiPose, the second section (8-10) show the effect of adding the bone length loss, the third section (11-14) shows results on the ``full'' (F) SkiPose for completeness. 
Results marked with an asterisk (*) are extended versions of main results reported in Table~\ref{tab:ski}. 
}
\label{tab:ablation_ski}
\end{table}
% }


==> tables/results_h36m_ski_sbs.tex <==
\begin{figure*}[t]
\begin{center}
\begin{minipage}{\columnwidth}
% \footnotesize
%< auto-adjusts font size to fill line
\inctabcolsep{-1pt} {
\captionof{table}{Human3.6M~\cite{todo}} \vspace{-1em}
\label{tab:h36m}
\resizebox{\linewidth}{!}{
\begin{tabular}{lc|cccc|c}\toprule
\multicolumn{2}{l}{\multirow{2}{*}{Method and supervision type}} & 
\multicolumn{2}{c}{PMPJPE$\downarrow$} & \multicolumn{2}{c}{NMPJPE$\downarrow$} &  \multirow{2}{*}{\stackanchor{$\Delta t$}{[s]}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & 4 & 2 & 4 & 2 \\
\midrule
\rowcolor[gray]{0.9}
Isakov et al. \cite{iskakov2019learnable} & \textbf{3D} & 20 & - & - & - & - \\ 
\midrule
AniPose \cite{karashchuk2020anipose} {\color{red} w/ GT} & S & 75 & 167 & 103 & 230 & 7 \\
Rhodin et al. \cite{rhodin2018skipose} & 2/3D & 65 & - & 80 & - & - \\
CanonPose \cite{wandt2020canonpose} & S & 53 & - & 82 & - & - \\
EpipolarPose (EP) \cite{kocabas2019epipolar} & S & 71 & - & 78 & - & - \\
Iqbal et al. \cite{iqbal2020weakly} & 2D & 55 & - & 66 & - & - \\
\midrule
% :EP~\cite{kocabas2019epipolar}
\textbf{MetaPose} (S1) & S & 74 & 87 & 83 & 95 & 0.2 \\
\textbf{MetaPose} (S1+S2) & 2D & \textbf{32} & \textbf{44} & \textbf{49} & \textbf{55} & 0.3 \\
% \midrule
% \textbf{MetaPose} (S1+S2/GD) & S & 43 & 66 & 53 & 75 & {\color{red} \textbf{2}} \\
% \textbf{MetaPose} (S1+S2/SS) & S & 39 & 50 & 56 & 63 & 0.3 \\
\bottomrule
\end{tabular}
}}
\end{minipage}
% ------------------------------------------------------------------
% ------------------------------------------------------------------
\hfill
% ------------------------------------------------------------------
% ------------------------------------------------------------------
\begin{minipage}{\columnwidth}
\inctabcolsep{-1pt} {
\captionof{table}{SkiPose-PTZ~\cite{todo}} \vspace{-1em}
\label{tab:ski}
\resizebox{\linewidth}{!}{
\begin{tabular}{lc|cccc|c}\toprule
\multicolumn{2}{l}{\multirow{2}{*}{Method and supervision type}} & 
\multicolumn{2}{c}{PMPJPE$\downarrow$} & \multicolumn{2}{c}{NMPJPE$\downarrow$} &  \multirow{2}{*}{\stackanchor{$\Delta t$}{[s]}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & 6 & 2 & 6 & 2 \\
\midrule
\\
\midrule
AniPose \cite{karashchuk2020anipose} {\color{red} w/ GT} & S & 50 & 62 & 221 & 273 & 7 \\
Rhodin et al. \cite{rhodin2018skipose} & 2/3D & - & - & 85 & - & - \\
CanonPose (CP) \cite{wandt2020canonpose} & S & 90 & - & 128 & - & - \\
\\
\\
\midrule
% CP~\cite{wandt2020canonpose}
\textbf{MetaPose} (S1) & S & 81 & 86 & 140 & 144 & 0.3 \\
\textbf{MetaPose} (S1+S2) & 2D & 42 & \textbf{50} & \textbf{53} & \textbf{59} & 0.4 \\
% \midrule
% \textbf{MetaPose} (S1+S2/GD) & S & \textbf{30} & 77 & 54 & 94 & {\color{red} \textbf{3}} \\
% \textbf{MetaPose} (S1+S2/SS) & S & 42 & 95 & 59 & 102 & 0.4 \\
\bottomrule
\end{tabular}
}}
\end{minipage}
\end{center}
\vspace{-1em}
% 
\captionof{figure}{
\textbf{Quantitative evaluation} --
Performance of different methods with \textit{four and two cameras} on Human3.6M and SkiPose-PTZ, Procrustes and Normalized MPJPE in millimeters, and inference time, supervision signal used \textit{during training}: 2D - ground truth 2D keypoints, 3D - ground truth 3D poses, S - self-supervision (i.e. using a pose estimation network pre-trained on a different dataset), 2/3D - 2D keypoint data with 3D poses on few subjects. 
% Top sections contains results reported in prior work, the bottom section contains our results. \AT{nobody cares about this!!!}
% \AT{The last two rows should NOT be in this table -- they meddle the story!
% These are ablations, so you are allow to run them on whatever you want, pull the last two rows out in their own table, and only do it for H36 so to avoid idiotic reviewers. TL;DR keep the story simple and the conclusions immediate to take.}
% \AT{p.s. why EP, and MetaPose/EP do not match? This is also confusing}
% \AT{I broke table spacing, sorry :P}
% \BU{done TODOs, but I still think that the vertically stacked Table \ref{tab:quantitative_extended} without holes looks better.}
}
\label{fig:quantitative}
\end{figure*}

==> tables/results_h36m_ski_with_sup.tex <==
\begin{table}[t]
\begin{center}
\inctabcolsep{-2.3pt} {
\begin{tabular}{lc|cccc|c}\toprule
\multicolumn{2}{l}{\multirow{2}{*}{Method and supervision type}} & 
\multicolumn{2}{c}{PMPJPE$\downarrow$} & \multicolumn{2}{c}{NMPJPE$\downarrow$} &  \multirow{2}{*}{\stackanchor{$\Delta t$}{[s]}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & 4 & 2 & 4 & 2 \\
\midrule
\rowcolor[gray]{0.9}
Isakov et al. \cite{iskakov2019learnable} & \textbf{3D} & 20 & - & - & - & - \\ 
\midrule
AniPose \cite{karashchuk2020anipose} w/ GT & S & 75 & 167 & 103 & 230 & 7 \\
Rhodin et al. \cite{rhodin2018skipose} & 2/3D & 65 & - & 80 & - & - \\
CanonPose \cite{wandt2020canonpose} & S & 53 & - & 82 & - & - \\
EpipolarPose (EP) \cite{kocabas2019epipolar} & S & 71 & - & 78 & - & - \\
Iqbal et al. \cite{iqbal2020weakly} & 2D & 55 & - & 66 & - & - \\
\midrule
% :EP~\cite{kocabas2019epipolar}
\textbf{MetaPose} (S1) & S & 74 & 87 & 83 & 95 & 0.2 \\
\textbf{MetaPose} (S1+S2) & 2D & \textbf{32} & \textbf{44} & \textbf{49} & \textbf{55} & 0.3 \\
% \midrule
\bottomrule
\end{tabular}

\bigskip
\begin{tabular}{lc|cccc|c}\toprule
\multicolumn{2}{l}{\multirow{2}{*}{Method and supervision type}} & 
\multicolumn{2}{c}{PMPJPE$\downarrow$} & \multicolumn{2}{c}{NMPJPE$\downarrow$} &  \multirow{2}{*}{\stackanchor{$\Delta t$}{[s]}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & 6 & 2 & 6 & 2 \\
\midrule
AniPose \cite{karashchuk2020anipose} w/ GT & S & 50 & 62 & 221 & 273 & 7 \\
Rhodin et al. \cite{rhodin2018skipose} & 2/3D & - & - & 85 & - & - \\
CanonPose (CP) \cite{wandt2020canonpose} & S & 90 & - & 128 & - & - \\
\midrule
% CP~\cite{wandt2020canonpose}
\textbf{MetaPose} (S1) & S & 81 & 86 & 140 & 144 & 0.3 \\
\textbf{MetaPose} (S1+S2) & 2D & 42 & \textbf{50} & \textbf{53} & \textbf{59} & 0.4 \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-1em}
% 
\captionof{figure}{
\textbf{Quantitative evaluation} --
Performance of different methods with \textit{four and two cameras} on Human3.6M and SkiPose-PTZ, Procrustes and Normalized MPJPE in millimeters, and inference time, supervision signal used \textit{during training}: 2D - ground truth 2D keypoints, 3D - ground truth 3D poses, S - self-supervision (i.e. using a pose estimation network pre-trained on a different dataset), 2/3D - 2D keypoint data with 3D poses on few subjects. 
}
\label{tab:quantitative_extended}
\end{table}

==> tables/sup_equiv_mlp.tex <==
\begin{table*}[]
\begin{tabular}{llllllll}
\textbf{Method} & \textbf{Loss} & \textbf{Model} & \textbf{2d} & \textbf{init} & \multicolumn{1}{r}{\textbf{4}} & \multicolumn{1}{r}{\textbf{3}} & \multicolumn{1}{r}{\textbf{2}} \\
Metapose & proj, teach & equiv & HT & EP & 38 & 45 & 45 \\
Metapose & proj & equiv & HT & EP & 32 & 39 & 44 \\
Metapose & proj, teach & MLP & HT & EP & 38 & 44 & 44 \\
Metapose & proj & MLP & HT & EP & 30 & 35 & 41
\end{tabular}
\caption{Eqvivariant-vs-MLP.\label{tab:equiv_mlp}}
\end{table*}

==> tables/sup_notation.tex <==
\begin{table}
\begin{center}

\inctabcolsep{-2pt} {
\begin{tabular}{cl}\toprule
$0 \leq t \leq T$ & timestamp $t$ \\
$0 \leq c \leq C$ & camera $c$ \\
$0 \leq k \leq K$ & joint $k$ \\
$0 \leq r \leq R$ & mixture component $r$ \\
$\bm{x}^{(t, c)}$ & input image \\
$\bm{q}^{(t, c)}$ & GT 2D pose \\
$\mathcal D = \{(\bm{x}^{(t, c)}, \bm{q}^{(t, c)})\}$ & trainig dataset \\
$\bm{y}$ & joint 3D pose and camera guess \\
$\bm{y} = (\bm{p}, \{\bm{e}^{(c)}\})$ & (3D pose, cameras' parameters) \\
$\bm{y}_{\text{init}}, \bm{y}_{\text{ref}}, \bm{y}_{\text{neur}}$ & initial, refined and neural estimates \\
$\pi^{(c)}(\bm{y}) = \pi(\bm{p}, \bm{e}^{(c)})$ & projection of $\bm{p}$ onto camera $c$ \\
$\bm{g} = \{(\bm{\mu}_r, \sigma_r, w_r)\}$ & Gaussian mixture parameters \\
$\bm{e}^{(c)} = (R^{(c)}, \bm{t}^{(c)}, s^{(c)})$ & weak projection parameters \\

$\bm{\tilde p}^{(c)}$ & monocular 3D pose estimate \\
\bottomrule
\end{tabular}
}\vspace*{-7px}
\end{center}
% \AS{Single notatiotn per row makes it less dense}
\caption{\textbf{Notation used in Method Section}.}
\label{tab:not}
\end{table}

==> tables/sup_rand_gt_init.tex <==
\begin{table}[]
\begin{tabular}{llllllll}
\textbf{Method} & \textbf{Loss} & \textbf{Model} & \textbf{2d} & \textbf{init} & \textbf{4} & \textbf{3} & \textbf{2} \\
AniPose & - & - & mHT & GT & 75 & 106 & 167 \\
AniPose & - & - & GT & GT & 0.3 & 0.5 & 2.7 \\
AniPose & - & - & mHT & rand & 198 & 215 & 269 \\
AniPose & - & - & GT & rand & 154 & 153 & 245 \\
Iterative & logp & - & HT & rand & 200 & 283 & 386 \\
Iterative & logp & - & HT & GT & 40 & 49 & 48 \\
Iterative & logp & - & GT & EP & 17 & 20 & 24 \\
Iterative & logp & - & GT & GT & 14 & 16 & 20
\end{tabular}
\caption{Random and GT init\label{tab:rand_gt_init}}
\end{table}

==> z_todo_macro.tex <==
\definecolor{blueish}{rgb}{0.0, 0.3, .6}
\newcommand{\at}[1]{{\color{blueish}#1}}
\newcommand{\At}[1]{\marginpar{\tiny{\textcolor{blueish}{#1}}}}
\newcommand{\AT}[1]{{\color{blueish}{\bf [AT: #1]}}}
\newcommand{\AS}[1]{{\color{olive}{\bf [AS: #1]}}}
\newcommand{\as}[1]{{\color{olive}{#1}}}
\newcommand{\BU}[1]{{\color{teal}{\bf [BU: #1]}}}
\newcommand{\bu}[1]{{\color{teal}{#1}}}
\newcommand{\todo}[1]{{\bf \color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\QUESTION}[1]{{\color{blue} //#1//}}
\newcommand{\todocite}{{\color{red} [cite] }}
\newcommand{\todocitex}[1]{{\color{red} $[$#1$]$ }}

